OFDM-RSMA: Robust Transmission under Inter-Carrier Interference

Rate-splitting multiple access (RSMA) is a multiple access scheme to mitigate the effects of the multi-user interference (MUI) in multi-antenna systems. In this study, we leverage the interference management capabilities of RSMA to tackle the issue of inter-carrier interference (ICI) in orthogonal frequency division multiplexing (OFDM) waveform. We formulate a sum-rate maximization problem to find the optimal subcarrier and power allocation for downlink transmission in a two-user system using RSMA and OFDM. A weighted minimum mean-square error (WMMSE)-based algorithm is proposed to obtain a solution for the formulated non-convex problem. We show that the marriage of rate-splitting (RS) with OFDM provides complementary strengths to cope with peculiar characteristic of wireless medium and its performance-limiting challenges including inter-symbol interference (ISI), MUI, ICI, and inter-numerology interference (INI). The sum-rate performance of the proposed OFDM-RSMA scheme is numerically compared with that of conventional orthogonal frequency division multiple access (OFDMA) and OFDM-non-orthogonal multiple access (NOMA). It is shown that the proposed OFDM-RSMA outperforms OFDM-NOMA and OFDMA in diverse propagation channel conditions owing to its flexible structure and robust interference management capabilities.

==> acros.tex <==
\usepackage{etoolbox}
\makeatletter
\newif\ifAC@uppercase@first%
\def\Aclp#1{\AC@uppercase@firsttrue\aclp{#1}\AC@uppercase@firstfalse}%
\def\AC@aclp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acl{#1}s%
	\fi%
}%
\def\Acp#1{\AC@uppercase@firsttrue\acp{#1}\AC@uppercase@firstfalse}%
\def\AC@acp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@ac{#1}s%
	\fi%
}%
\def\Acfp#1{\AC@uppercase@firsttrue\acfp{#1}\AC@uppercase@firstfalse}%
\def\AC@acfp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acf{#1}s%
	\fi%
}%
\def\Acsp#1{\AC@uppercase@firsttrue\acsp{#1}\AC@uppercase@firstfalse}%
\def\AC@acsp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acs{#1}s%
	\fi%
}%
\edef\AC@uppercase@write{\string\ifAC@uppercase@first\string\expandafter\string\MakeUppercase\string\fi\space}%
\def\AC@acrodef#1[#2]#3{%
	\@bsphack%
	\protected@write\@auxout{}{%
		\string\newacro{#1}[#2]{\AC@uppercase@write #3}%
	}\@esphack%
}%
\def\Acl#1{\AC@uppercase@firsttrue\acl{#1}\AC@uppercase@firstfalse}
\def\Acf#1{\AC@uppercase@firsttrue\acf{#1}\AC@uppercase@firstfalse}
\def\Ac#1{\AC@uppercase@firsttrue\ac{#1}\AC@uppercase@firstfalse}
\def\Acs#1{\AC@uppercase@firsttrue\acs{#1}\AC@uppercase@firstfalse}
\robustify\Aclp
\robustify\Acfp
\robustify\Acp
\robustify\Acsp
\robustify\Acl
\robustify\Acf
\robustify\Ac
\robustify\Acs
\makeatother

\acrodef{3GPP}{3rd Generation Partnership Project}
\acrodef{4-QAM}{4-state quadrature amplitude modulation}
\acrodef{4G}{fourth generation}
\acrodef{5G}{fifth generation}
\acrodef{6G}{sixth generation}
\acrodef{8-PSK}{8-state phase shift keying}
\acrodef{16-QAM}{16-state quadrature amplitude modulation}
\acrodef{64-QAM}{64-state quadrature amplitude modulation}
\acrodef{ACF}{auto-correlation function}
\acrodef{ACI}{adjacent channel interference}
\acrodef{ACLR}{adjacent channel leakage ratio}
\acrodef{ACPR}{adjacent channel power ratio }
\acrodef{ADC}{analog-to-digital converter}
\acrodef{ADSL}{asymmetric digital subscriber line}
\acrodef{AFH}{adaptive frequency hopping}
\acrodef{AIC}{Akaike information criteria}
\acrodef{AI}{Artificial Intelligence}
\acrodef{ALRT}{average likelihood ratio test}
\acrodef{AM}{amplitude modulation}
\acrodef{AoA}{angle-of-arrival}
\acrodef{AoD}{angle-of-departure}
\acrodef{AP}{access point}
\acrodef{ARQ}{automatic repeat request}
\acrodef{AR}{augmented reality}
\acrodef{AWGN}{additive white Gaussian noise}
\acrodef{AWMMSE}{augmented weighted minimum mean-square error}
\acrodef{BC}{broadcast channel}
\acrodef{BER}{bit-error-rate}
\acrodef{BE}{best effort service}
\acrodef{BLER}{block error rate}
\acrodef{BPF}{band pass filter}
\acrodef{BPSK}{binary phase shift keying}
\acrodef{BS}{base station}
\acrodef{BSA}{blind signal analysis}
\acrodef{BT}{bandwidth-time}
\acrodef{BW}{bandwidth}
\acrodef{BWA}{broadband wireless access}
\acrodef{CAD}{computer aided design}
\acrodef{CAF}{cyclic autocorrelation function}
\acrodef{CCDF}{complementary cumulative distribution function}
\acrodef{CCI}{co-channel interference}
\acrodef{CDF}{cumulative distribution function }
\acrodef{CDL}{clustered delay line}
\acrodef{CDMA}{code division multiple access }
\acrodef{CDMA}{code division multiple access}
\acrodef{CD-NOMA}{code-domain \ac{NOMA}}
\acrodef{CFC}{channel frequency correlation}
\acrodef{CFR}{channel frequency response}
\acrodef{CINR}{carrier-to-inteference-plus-noise ratio}
\acrodef{CIR}{channel impulse response}
\acrodef{CLT}{central limit theorem}
\acrodef{CMA}{constant modulus algorithm}
\acrodef{CNN}{convolutional neural networks}
\acrodef{CP}{cyclic prefix}
\acrodef{CPI}{coherent processing interval}
\acrodef{CRC}{cyclic redundancy check}
\acrodef{CRLB}{Cram\'er-Rao lower bound}
\acrodef{CR}{cognitive radio}
\acrodef{CSD}{cyclic spectral density}
\acrodef{CSIT}{channel state information at the transmitter}
\acrodef{CSI}{channel state information}
\acrodef{CSMA}{carrier sense multiple accessing}
\acrodef{CTS}{clear to send}
\acrodef{DAB}{digital audio broadcasting}
\acrodef{DAC}{digital-to-analog converter}
\acrodef{DC}{direct current}
\acrodef{DDC}{digital down conversion}
\acrodef{DFE}{decision feedback equalizer}
\acrodef{DFRC}{dual function radar communication}
\acrodef{DFS}{dynamic frequency selection}
\acrodef{DFT-S-OFDM}{DFT-Spread-OFDM}
\acrodef{DFT}{discrete Fourier transform}
\acrodef{DL}{deep learning}
\acrodef{DNN}{deep neural network}
\acrodef{DoF}{degrees of freedom}
\acrodef{DS-CDMA}{direct spread code division multiple access}
\acrodef{DSP}{digital signal processor}
\acrodef{DSSS}{direct-sequence spread-spectrum}
\acrodef{DUC}{digital up conversion}
\acrodef{DUT}{device under test}
\acrodef{DVB-T}{terrestrial digital video broadcasting}
\acrodef{DWT}{discrete wavelet transform}
\acrodef{ED}{energy detection}
\acrodef{EDGE}{enhanced data rates for GSM evolution}
\acrodef{EGC}{equal gain-combining}
\acrodef{EM}{electromagnetic}
\acrodef{MBB}{mobile broadband}
\acrodef{eMBB}{enhance mobile broadband}
\acrodef{EVM}{error vector magnitude}
\acrodef{FB}{feature-based}
\acrodef{FBMC}{filter bank multicarrier}
\acrodef{FCH}{frame control header}
\acrodef{FDD}{frequency division duplexing}
\acrodef{FEC}{forward error correction}
\acrodef{FER}{frame-error-rate}
\acrodef{FFT}{fast Fourier transform}
\acrodef{FHMA}{frequency hopped multiple access}
\acrodef{FHSS}{frequency-hopping spread spectrum}
\acrodef{FH}{frequency hopping}
\acrodef{FMCW}{frequency modulated continuous wave}
\acrodef{FPGA}{field-programmable gate array}
\acrodef{FSK}{frequency shift keying}
\acrodef{G-REM}{generalized radio environment monitoring}
\acrodef{GB}{grant based}
\acrodef{GFSK}{Gaussian frequency shift keying}
\acrodef{GF}{grant free}
\acrodef{GLRT}{generalized likelihood ratio test}
\acrodef{GMSK}{Gaussian minimum shift keying}
\acrodef{GNSS}{global navigation satellite system}
\acrodef{GoF}{goodness-of-fit}
\acrodef{GOS}{grade of service}
\acrodef{GPP}{general purpose processor}
\acrodef{GPS}{global positioning system}
\acrodef{GSM}{global system for mobile communications}
\acrodef{HMM}{hidden Markov model}
\acrodef{ICI}{inter-carrier interference}
\acrodef{IDFT}{inverse discrete Fourier transform}
\acrodef{IDMA}{interleave division multiple access}
\acrodef{IEEE}{institute of electrical and electronics engineers}
\acrodef{IFFT}{inverse fast Fourier transform}
\acrodef{IF}{intermediate frequencies}
\acrodef{IMD}{inter-modulation distortion}
\acrodef{INI}{inter-numerology interference}
\acrodef{IoT}{Internet of Things}
\acrodef{IP}{internet protocol}
\acrodef{I/Q}{in-phase and quadrature-phase}
\acrodef{ISI}{inter-symbol interference}
\acrodef{ITU}{International Telecommunication Union}
\acrodef{IUI}{inter-user interference}
\acrodef{JRC}{joint radar and communication}
\acrodef{KKT}{Karush-Kuhn-Tucker}
\acrodef{K-L}{Kullback-Leibler}
\acrodef{LAN}{local area network}
\acrodef{LCR}{level crossing rate}
\acrodef{LDPC}{low density parity coding}
\acrodef{LDS-MA}{low density spreading multiple access}
\acrodef{LFM}{linear frequency modulation}
\acrodef{LFSR}{linear feedback shift register}
\acrodef{LHS}{left-hand side}
\acrodef{LLR}{log-likelihood ratio}
\acrodef{LMMSE}{linear minimum mean-square error}
\acrodef{LMS}{least-mean-square}
\acrodef{LNA}{low noise amplifier}
\acrodef{LOS}{line-of-sight}
\acrodef{LO}{local oscillator}
\acrodef{LS}{least squares}
\acrodef{LSTM}{long short-term memory}
\acrodef{LTE}{long term evolution}
\acrodef{LTE-A}{\ac{LTE}-advanced}
\acrodef{LU}{licensed user}
\acrodef{LTV}{linear time-varying}
\acrodef{MA}{multiple accessing}
\acrodef{MACA}{multiple access collision avoidance}
\acrodef{MAC}{medium access control}
\acrodef{MAI}{multi access interference}
\acrodef{MANET}{Mobile Ad-Hoc Network}
\acrodef{MC-CDMA}{multi-carrier code division multiple access}
\acrodef{MCS}{modulation and coding scheme}
\acrodef{MCD}{measurement capable device}
\acrodef{MDL}{minimum descriptive length}
\acrodef{MI}{mutual information}
\acrodef{MIMO}{multiple-input multiple-output}
\acrodef{MISO}{multiple-input single-output}
\acrodef{MLE}{maximum likelihood estimation}
\acrodef{MLSE}{maximum likelihood sequence estimation}
\acrodef{MMSE}{minimum mean-square error}
\acrodef{mMIMO}{massive \ac{MIMO}}
\acrodef{mMTC}{massive machine type communication}
\acrodef{mmWave}{millimeter wave}
\acrodef{MPA}{message-passing algorithm}
\acrodef{MPC}{multipath component}
\acrodef{MSE}{mean-squared-error}
\acrodef{MSK}{minimum shift keying}
\acrodef{MS}{mobile station}
\acrodef{MU}{multi-user}
\acrodef{MUI}{multi-user interference}
\acrodef{MUST}{multi-user superposition transmission}
\acrodef{NBI}{narrow-band interference}
\acrodef{NBF}{narrow-band filter}
\acrodef{NGMA}{next generation wireless networks}
\acrodef{NLOS}{non-\ac{LOS}}
\acrodef{NOMA}{non-orthogonal multiple access}
\acrodef{NR}{new radio}
\acrodef{NTN}{non-terrestrial networks}
\acrodef{OFDM-CSMA}{OFDM carrier sense multiple accessing}
\acrodef{OFDM-FDMA}{OFDM frequency division multiple accessing}
\acrodef{OFDM-TDMA}{OFDM time division multiple accessing}
\acrodef{OFDMA}{orthogonal frequency division multiple access}
\acrodef{OFDM}{orthogonal frequency division multiplexing}
\acrodef{OMA}{orthogonal multiple access}
\acrodef{OQPSK}{offset quadrature phase‐shift keying}
\acrodef{OSI}{open systems interconnection reference}
\acrodef{OSR}{oversampling rate}
\acrodef{OTA}{over-the-air}
\acrodef{OTFS}{orthogonal time-frequency space}
\acrodef{PA}{power amplifier}
\acrodef{PAPR}{peak-to-average power ratio}
\acrodef{PDF}{probability density function}
\acrodef{PDMA}{pattern division multiple access}
\acrodef{PD-NOMA}{power-domain \ac{NOMA}}
\acrodef{PDP}{power delay profile}
\acrodef{PER}{packet-error-rate}
\acrodef{PHY}{physical layer}
\acrodef{PICR}{peak interference-to-carrier ratio}
\acrodef{PLS}{physical layer security}
\acrodef{PMF}{partial match-filtering}
\acrodef{PMP}{point to multi-point}
\acrodef{PN}{pseudo noise}
\acrodef{PPP}{Poisson point process}
\acrodef{PRBS}{pseudo-random binary sequence}
\acrodef{PRI}{pulse repetition interval}
\acrodef{PRF}{pulse repetition frequency}
\acrodef{PSD}{power spectral density}
\acrodef{PSK}{phase shift keying}
\acrodef{PTS}{partial transmit sequences}
\acrodef{PU}{primary user}
\acrodef{PUSC}{partially used sub-channeling}
\acrodef{QAM}{quadrature amplitude modulation}
\acrodef{QCQP}{quadratically constrained quadratic program}
\acrodef{QoS}{quality of service}
\acrodef{QPSK}{quadrature phase shift keying}
\acrodef{RACH}{random access channel}
\acrodef{RAT}{radio access technology}
\acrodef{RA}{reconfigurable antenna}
\acrodef{radar}{radio detection and ranging}
\acrodef{RCS}{radar-sensing and communication}
\acrodef{RC}{raised cosine}
\acrodef{REM}{radio environment map}
\acrodef{RF-REM}{radio frequency \ac{REM}}
\acrodef{RHS}{right-hand side}
\acrodef{RIS}{reconfigurable intelligent surface}
\acrodef{RL}{reinforcement learning}
\acrodef{RLS}{recursive least-squares}
\acrodef{RMS}{root mean squared}
\acrodef{ROC}{receiver operating characteristic}
\acrodef{RRC}{root raised cosine}
\acrodef{RS}{rate-splitting}
\acrodef{RSM}{range sidelobe modulation}
\acrodef{RSSI}{received signal strength indicator}
\acrodef{RTS}{request to send}
\acrodef{RT}{ray-tracing}
\acrodef{RU}{rental user}
\acrodef{RVC}{reverberation chamber}
\acrodef{Rx}{receiver}
\acrodef{SAW}{surface acoustic wave}
\acrodef{SC-FDE}{single carrier frequency domain equalization}
\acrodef{SC-FDMA}{single carrier frequency division multiple access}
\acrodef{SCMA}{sparse code multiple access}
\acrodef{SCS}{sub-carrier spacing}
\acrodef{SC}{superposition coding}
\acrodef{SCF}{spectral correlation function}
\acrodef{SDMA}{space-division multiple access}
\acrodef{SDR}{software defined radio}
\acrodef{SDU}{service data unit}
\acrodef{SE}{spectral efficiency}
\acrodef{SER}{symbol error rate}
\acrodef{SIC}{successive interference cancellation}
\acrodef{SINR}{signal-to-interference-plus-noise ratio}
\acrodef{SIR}{signal-to-interference ratio}
\acrodef{SISO}{single-input single-output}
\acrodef{SM}{selected mapping}
\acrodef{SNR}{signal-to-noise ratio}
\acrodef{SS}{subscriber station}
\acrodef{SR}{sum-rate}
\acrodef{STC}{space time coding}
\acrodef{STDCC}{swept time-delay cross correlation}
\acrodef{STFT}{short time Fourier transform}
\acrodef{SVD}{singular value decomposition}
\acrodef{SU}{secondary user}
\acrodef{TDD}{time division duplexing}
\acrodef{TDL}{tapped delay line}
\acrodef{TDMA}{time division multiple access}
\acrodef{TFA}{time-frequency analysis}
\acrodef{TH}{time hopping}
\acrodef{TP}{transmission point}
\acrodef{TVWS}{television white space}
\acrodef{Tx}{transmitter}
\acrodef{UAV}{unmanned aerial vehicles}
\acrodef{UE}{user equipment}
\acrodef{UMTS}{universal mobile telecommunications service}
\acrodef{URLLC}{ultra reliable, low latency communication}
\acrodef{USRP}{universal software radio peripheral}
\acrodef{UWB}{ultra wide band}
\acrodef{V2V}{vehicle-to-vehicle}
\acrodef{VANET}{vehicular ad-hoc network}
\acrodef{VCO}{voltage-controlled oscillator}
\acrodef{VNA}{vector network analyzer}
\acrodef{VR}{virtual reality}
\acrodef{VSA}{vector signal analyser}
\acrodef{VSG}{vector signal generator}
\acrodef{WCDMA}{wideband \ac{CDMA}}
\acrodef{Wi-Fi}{wireless fidelity}
\acrodef{WiMAX}{worldwide interoperability for microwave access}
\acrodef{WLAN}{wireless local area network}
\acrodef{WMAN}{wireless metropolitan area network}
\acrodef{WMMSE}{weighted \ac{MMSE}}
\acrodef{WPAN}{wireless personal area network}
\acrodef{WRAN}{wireless regional area network}
\acrodef{WSSUS}{wide-sense stationary uncorrelated scattering}
\acrodef{WSS}{wide-sense stationary}
\acrodef{WSR}{weighted sum-rate}
\acrodef{WT}{wavelet transform}
\acrodef{XPR}{cross polarization power ratio}
\acrodef{ZPSK}{zero-padded phase shift keying}
\acrodef{FDMA}{frequency division multiple accessing}
\acrodef{DRX}{discontinuous reception}
\acrodef{MNO}{mobile network operator}
\acrodef{GPU}{graphics processing unit}
\acrodef{RLC}{radio link control} 
\acrodef{PDCP}{packet data convergence protocol} 
\acrodef{BBU}{baseband unit} 
\acrodef{RRH}{remote radio head} 
\acrodef{ADT}{abstract data type} 
\acrodef{RSMA}{rate-splitting multiple access} 

%%%%% Conflicting Acronyms %%%%%%%%%
\acrodef{ML}{machine learning}
% \acrodef{ML}{maximum likelihood}
% \acrodef{CW}{carrier wave}
\acrodef{CW}{continuous wave}
\acrodef{RF}{radio frequency}
\acrodef{DTFT}{discrete-time Fourier transform}
\acrodef{PLL}{phase-locked loop}
\acrodef{OOBE}{out-of-band emission}
\acrodef{FDE}{frequency domain equalization}
\acrodef{ZP}{zero-padding}
\acrodef{AFC}{adaptive frequency correction}
\acrodef{SPNIR}{signal-to-phase-noise-interference-ratio}
\acrodef{AM-AM}{amplitude-to-amplitude}
\acrodef{AM-PM}{amplitude-to-phase}
\acrodef{TDM}{time division multiplexing}
\acrodef{QCQP}{quadratically constrained quadratic program}
\acrodef{SOCP}{second-order
cone program}
\acrodef{GP}{geometric program}
\acrodef{SDP}{semidefinite program}
\acrodef{LMI}{linear matrix inequality}

